A Study of Multimodal Person Verification Using Audio-Visual-Thermal Data

In this paper, we study an approach to multimodal person verification using audio, visual, and thermal modalities. The combination of audio and visual modalities has already been shown to be effective for robust person verification. From this perspective, we investigate the impact of further increasing the number of modalities by adding thermal images. In particular, we implemented unimodal, bimodal, and trimodal verification systems using state-of-the-art deep learning architectures and compared their performance under clean and noisy conditions. We also compared two popular fusion approaches based on simple score averaging and the soft attention mechanism. The experiment conducted on the SpeakingFaces dataset demonstrates the superior performance of the trimodal verification system. Specifically, on the easy test set, the trimodal system outperforms the best unimodal and bimodal systems by over 50% and 18% relative equal error rates, respectively, under both the clean and noisy conditions. On the hard test set, the trimodal system outperforms the best unimodal and bimodal systems by over 40% and 13% relative equal error rates, respectively, under both the clean and noisy conditions. To enable reproducibility of the experiment and facilitate research into multimodal person verification, we made our code, pretrained models, and preprocessed dataset freely available in our GitHub repository.

==> Odyssey 2022 Latex Template/1_intro.tex <==
%What is the goal and motivation of this paper?
% This work addresses the multimodal person verification using audio, visual, and thermal modalities.
Person verification is the general task of verifying a person's identity using various biometric characteristics.
The two widely used biometric features are voice (i.e., audio) and face (i.e., visual), corresponding to the speaker~\cite{DBLP:journals/spm/HansenH15} and the face~\cite{DBLP:conf/sibgrapi/Masi0HN18} verification tasks, respectively.
%Recently, it was observed that the combination of audio and visual modalities yields more accurate and robust person verification system [cite].
Recently, it has been observed that the combination of audio and visual modalities positively impacts the person verification task, yielding more accurate and robust systems~\cite{shon2019noise,qian2021audio}.
Presumably, increasing the number of modalities with the use of thermal images might boost the performance of a person verification system.

%Background info. Is there any work that used audio, visual and thermal modalities for person verification?
To date, most of the existing works on person verification have focused on unimodal approaches utilizing various biometric features, such as voice, face, fingerprints, iris, gait, and so on~\cite{minaee2019biometrics}.
%The most popular ones are voice~\cite{dehak2010front,snyder2018x,nagrani2020voxceleb} and face~\cite{DBLP:conf/bmvc/ParkhiVZ15,DBLP:conf/cvpr/SchroffKP15} biometrics, where remarkable progress has been achieved.
Remarkable progress has been achieved in the use of voice~\cite{dehak2010front,DBLP:conf/interspeech/SnyderGPK17,nagrani2020voxceleb} and face~\cite{DBLP:conf/bmvc/ParkhiVZ15,DBLP:conf/cvpr/SchroffKP15} biometrics.
However, the performance of unimodal verification systems degrades substantially under challenging conditions~\cite{shon2019noise,qian2021audio}.
%Despite remarkable progress of unimodal verification systems, their performance significantly drops under the more challenging conditions~\cite{qian2021audio}.
In response, several works have turned to multimodal approaches that introduce effective audio-visual fusion strategies.
For example,~\cite{DBLP:conf/icassp/SellDSEG18,alam2020analysis} combined the scores generated by unimodal verification systems.
In contrast,~\cite{shon2019noise,qian2021audio} explored fusion strategies using attention-based deep neural networks~\cite{DBLP:journals/corr/BahdanauCB14} and found that the proposed multimodal verification systems outperformed their unimodal counterparts and were more robust to noise.
%To further facilitate research into multimodal person verification, several multimedia datasets have been introduced \cite{DBLP:conf/icassp/SellDSEG18,nagrani2017voxceleb,chung2018voxceleb2}, and challenges have been organized~\cite{sadjadi20202019}.
 
%Why thermal modality?
Recently, consumer electronics manufacturers have started to equip smartphones with thermal cameras~\cite{one_pro,s62}, bringing to market mobile devices that incorporate the triplet of audio, visual, and thermal modalities.
A thermal camera presents new opportunities for a wide range of applications. %, including person verification.
%A thermal camera introduces new opportunities for a wide range of applications, including human–computer interaction (HCI), biometric authentication, and recognition systems.
In particular, it enables a more nuanced analysis of images in suboptimal physical environments (e.g., nighttime) and reduces the effects of variation in background, clothing, accessories, and appearance (e.g., makeup and contact lenses).
%In particular, it enables a more nuanced analysis of multi-modal person recognition systems in suboptimal physical environments (e.g., at night), and in extreme cases of corruption, failure or missing data on either modality.
Additionally, a high-resolution thermal camera can provide more granular association of temperature values with facial features.
Its combination with other modalities can potentially strengthen multimodal person verification systems, by providing complementary information and alleviating the respective drawbacks of other modalities. 
Thermal images have been successfully deployed for speech recognition~\cite{DBLP:journals/tce/AndersonFT13}, lip reading~\cite{saitoh2006lip}, and person recognition using body images~\cite{DBLP:journals/sensors/NguyenHKP17}. 

%Contribution of this paper
In this work, we investigate whether the addition of thermal images as a third modality can improve the performance (accuracy and robustness) of audio-visual person verification systems. 
To the best of our knowledge, this is the first attempt at audio-visual-thermal person verification.
In particular, we adapted the SpeakingFaces dataset~\cite{abdrakhmanova2021speakingfaces} to the trimodal person verification task and shared the preprocessed data with the community.
%Additionally, we developed unimodal, bimodal (i.e., audio-visual) and trimodal (i.e., audio-visual-thermal) verification systems using the state-of-the-art deep learning architectures, and assessed their performance under different conditions, such as clean and noisy data.
We also developed unimodal, bimodal (i.e., audio-visual) and trimodal (i.e., audio-visual-thermal) verification systems using state-of-the-art deep learning architectures based on ResNet34~\cite{DBLP:conf/cvpr/HeZRS16}.
Additionally, we compared two popular fusion strategies based on simple score averaging~\cite{DBLP:conf/avbpa/LuceyC03,DBLP:conf/icassp/SellDSEG18} and the attention mechanism~\cite{DBLP:journals/corr/BahdanauCB14}.
%, and found the score averaging to perform better. 

We prepared two evaluation sets denoted as \textit{easy} and \textit{hard}, where the latter consists only of same gender pairs, and evaluated all models under two data conditions: 
%1) \textit{train clean / evaluation clean}, meaning train, validation and test sets did not contain any augmentations or noise, 2) \textit{train noisy / evaluation noisy}, where each of the three sets contained $30\%$ of noise.
\begin{itemize}
    \item[1)] \textit{Clean:} The training, validation, and test sets contained no augmentations or noise.
    \item[2)] \textit{Noisy:} Each of the three sets contained $30\%$ noise.
\end{itemize}


%Additionally, we prepared two evaluation sets denoted as \textit{easy} and \textit{hard}, where the latter consists only of same gender pairs.
%three conditions: 1) \textit{train clean / evaluation (i.e., validation and test sets) clean}, 2) \textit{train clean / evaluation noisy}, and 3) \textit{train noisy / evaluation noisy}.
%two conditions: 1) \textit{train clean / evaluation (i.e., validation and test sets) clean}, 2)  \textit{train noisy / evaluation noisy}.
%We also compared two popular fusion strategies based on simple score averaging and attention mechanism.

Experimental results on the \textit{easy} test set show that under the clean and noisy conditions the trimodal verification system outperforms the best unimodal system by 56\% and 51\% relative equal error rates (EERs), respectively.
The improvements over the best bimodal system under both conditions are over 18\% relative EERs.
On the \textit{hard} test set, the relative EER improvements under the clean and noisy conditions by the trimodal system over the best unimodal system are 52\% and 42\%, respectively.
The improvements over the best bimodal system are 18\% and 12\% relative EERs under the clean and noisy conditions, respectively.

%, and achieves similar results under the condition 2).
%Experiment results showed that in clean condition the trimodal verification system outperforms the audio-visual system by 18\% relative equal error rate (EER).
%In noisy condition, the trimodal system achieved 28\% relative EER improvement over the audio-visual systems.

The main contributions of our work are as follows:
\begin{itemize}
    \item[1)] We developed a trimodal person verification system based on audio-visual-thermal streams using state-of-the-art neural network architectures, and compared it with unimodal and bimodal systems.
    \item[2)] We evaluated the performance of the trimodal system under the clean and noisy conditions, and assessed the efficacy of two different fusion strategies. 
    \item[3)] We prepared an audio-visual-thermal dataset to facilitate research on multimodal person verification in this direction.
    \item[4)] We made our code, pretrained models, and dataset freely available$^{\ref{ft:github}}$ to enable experiment reproducibility.
    %\item[4)] We made our code, pretrained models, and dataset freely available\footnote{\url{https://github.com/IS2AI/trimodal_person_verification}\label{ft:github}} to enable experiment reproducibility.
\end{itemize}

The rest of the paper is organized as follows:
Section~\ref{sec:related} briefly reviews related work on person verification.
Section~\ref{sec:dataset} details the specifications of the SpeakingFaces dataset used in our experiments.
Section~\ref{sec:method} describes the architecture of the developed person verification systems.
Section~\ref{sec:exp_setup} presents the experimental setup. Section~\ref{sec:exp_results} discusses the obtained results. Section~\ref{sec:conclusion} concludes the paper and  highlights directions for future work.



\iffalse
The main contributions are:
\begin{itemize}
    \item We  introduce  a  multimodal  person  verification  system  that  utilizes  three data streams: thermal, visual and audio.
    \item We analyze the effect of each stream in optimal and suboptimal conditions.
    \item We explore different combinations of data sources.
\end{itemize}

Recently, a global smartphone market started to receive new smartphones equipped with thermal cameras~\cite{abdrakhmanova2021speakingfaces}, which if utilized correctly can open new opportunities. 
For example, the fusion of audio, visual and thermal data streams introduce new opportunities for multimodal data use in a wide range of applications, including human–computer interaction (HCI), biometric authentication, and recognition systems. 
A high-resolution thermal camera can facilitate an association of temperature values with facial features, and its combination with other streams can further strengthen multimodal systems by alleviating respective drawbacks of each individual stream. In particular, the composition of the three streams enables a more nuanced analysis of multimodal systems in applications such as person recognition in suboptimal physical environments (e.g.,at night), and in extreme cases of corruption, failure or missing data on either modality. %[given that phones now have thermal cameras it makes sense to consider it as a another source of biometric authentication] 
With the increasing popularity of biometric authentication in personal devices such as phones and computers (give examples), and in private entities such as vehicles and house/office buildings, robust person recognition systems become of paramount importance. 
\fi 






==> Odyssey 2022 Latex Template/2_related.tex <==
%VERSION 1
With the increasing popularity of biometric authentication in personal devices (e.g., mobile phones, tablets, computers, etc.), and in private entities (e.g., vehicles, houses, offices, etc.), robust and reliable person verification has become of paramount importance~\cite{bhattacharyya2009biometric}.
In recent years, many effective verification approaches have been proposed where promising results have been achieved~\cite{DBLP:journals/access/RuiY19}.
These approaches utilize various biometric features, including voice, face, fingerprint, palmprint, iris, and gait, to name a few.
Among the aforementioned biometrics, voice and face recognition has attracted substantial research interest in the academic community.


\subsection{Speaker verification}
Speaker verification aims to verify a person’s claimed identity using voice biometrics.
With the growing popularity of deep neural network (DNN), the leading modeling approach for speaker verification has transferred from the traditional Gaussian Mixture Model-Universal Background Model (GMM-UBM)~\cite{reynolds2000speaker} and \textit{i}-vector~\cite{dehak2010front} to deep speaker embedding representation learning.
A typical speaker embedding learning approach is \textit{d}-vector~\cite{variani2014deep}, where a fully-connected DNN is used to extract frame-level deep features.
These features are then averaged to form an utterance-level speaker representation.
%A typical speaker embedding learning approach is \textit{d}-vector~\cite{variani2014deep}, where an utterance-level speaker representation is obtained by averaging the frame-level deep features.
Another popular speaker embedding learning approach is the time-delay neural network (TDNN) based \textit{x}-vector~\cite{DBLP:conf/interspeech/SnyderGPK17}, which has been shown to achieve state-of-the-art results in multiple datasets~\cite{snyder2018x}.
Recently, more advanced neural architectures, such as ResNet34, have been shown to further improve performance by extracting \textit{r}-vectors~\cite{zeinali2019but}.
In this work, we also employed ResNet34 to learn speaker embedding vectors from the audio stream.


\subsection{Face verification}
Face verification aims to verify a person’s claimed identity using visual images.
Since the impressive success of the AlexNet~\cite{DBLP:conf/nips/KrizhevskySH12} architecture in the ImageNet competition, deep convolutional neural network (DCNN)-based approaches have become the mainstream for the face verification task.
For example, DeepFace~\cite{taigman2014deepface} achieved human-level performance on the challenging LFW benchmark~\cite{LFWTech} for the first time.
Furthermore, in recent years, researchers have explored many different DCNN-based architectures for the face verification task, where remarkable improvements have been achieved.
These architectures include, but not limited to, DeepID~\cite{sun2015deepid3}, VGGNet~\cite{DBLP:journals/corr/SimonyanZ14a}, FaceNET~\cite{DBLP:conf/cvpr/SchroffKP15}, and ResFace~\cite{DBLP:conf/cvpr/HeZRS16}.
In our work, we will employ ResNet34 to extract embedding vectors from both visual and thermal images.

%Especially, multi-modal person verification based on audio and visual signals start to gain popularity attracting more and more research interest~\cite{shon2019noise,qian2021audio}.


\subsection{Audio-visual person verification}
Although speaker verification and face verification have achieved remarkable progress in recent years, their performance decreases significantly under more challenging conditions.
For example, speaker verification is sensitive to changes in acoustic characteristics due to background noise, the person's mood (e.g., happy, angry, etc.), the uttered text, the recording device, distance, and so on.
Similarly, the performance of face verification is vulnerable to illumination, pose, emotion, distance.

To alleviate the drawbacks of the two verification approaches, researchers are turning to audio-visual verification approaches utilizing both modalities.
The initial work in this direction employed score-level fusion strategies~\cite{DBLP:conf/icassp/SellDSEG18,alam2020analysis,DBLP:conf/clear/LuqueMGAFMMMVH06}, where scores obtained from separately trained unimodal models were combined.
More recent works exploit attention-based fusion~\cite{shon2019noise,qian2021audio} to judiciously combine salient features from input modalities.
Overall, compared to unimodal verification systems, multimodal systems have been shown to be more accurate and robust, especially under noisy conditions.

To facilitate research on audio-visual person verification, various multimedia datasets have been introduced, such as VAST~\cite{DBLP:conf/lrec/TraceyS18}, JANUS~\cite{DBLP:conf/icassp/SellDSEG18}, VoxCeleb 1~\cite{nagrani2017voxceleb} \& 2~\cite{chung2018voxceleb2}.
Additionally, several person verification challenges have been organized~\cite{DBLP:conf/clear/StiefelhagenBBGMS06,sadjadi20202019}.
For example, the 2019 NIST speaker recognition evaluation (SRE) challenge~\cite{sadjadi20202019} proposed to use visual information in conjunction with audio recordings to increase the robustness of verification systems.
As a result, audio-visual fusion was found to result in remarkable performance gains (more than 85\% relative) over audio-only or face-only systems.
%Thanks to the aforementioned efforts, many interesting audio-visual person verification approaches were proposed.
In this paper, we will investigate further increase of modalities by supplementing an audio-visual system with thermal images.
%Among them, the most widely used datasets are VoxCeleb 1 \& 2.
%The VoxCeleb 1 contains around 1,200 speakers uttering over 150,000 recordings, and it is usually used as an evaluation set.
%The VoxCeleb 2 contains around 6,000 speakers uttering over 1 million recordings, and it is usually used as a training set.
%Other datasets where both modalities are present, and thus, can potentially support the audio-visual research  are~\cite{DBLP:journals/ivc/EveringhamSZ09,DBLP:conf/cvpr/OrtizWS13,DBLP:conf/icassp/SchmidtSM14}. 

%Additionally, to further facilitate the audio-visual person verification research, 2019 NIST speaker recognition evaluation (SRE) challenge proposed to use visual information in conjunction with the audio recordings to increase robustness of verification systems~\cite{sadjadi20202019}.
%As a result of challenge, many interesting audio-visual person verification approaches were proposed~\cite{alam2020analysis} [cite].

%Up to date, many effective audio-visual person verification approaches have been proposed.
%Depending on the level where the fusion is conducted, multi-modal approaches can be categorized into three main types: 1) feature-level, 2) embedding-level, and 3) score-level fusion.
%In the feature-level fusion, bla-bla.
%In the embedding-level fusion, bla-bla.
%Lastly, in the score-level fusion, bla-bla.





\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%VERSION 2
Person verification has been an active field of research for several decades~\cite{zhang2017end, snyder2018x, taigman2014deepface, wen2016discriminative}. Many approaches that have been already proposed are based on a single-stream framework, which is either on a person's voice or on his or her facial appearance, and many of them evolved over time. For example, the approaches for speaker recognition started from traditional probabilistic approaches~\cite{reynolds2000speaker, dehak2010front} and moved to deep speaker embedding ones~\cite{variani2014deep, snyder2017deep}. Whereas the approaches for face recognition have transferred from local descriptors based learning~\cite{cao2010face, lei2013learning} to deep convolutional neural networks~\cite{krizhevsky2012imagenet, parkhi2015deep, schroff2015facenet}.



Although single modality person recognition showed competitive performance, it was inferred that multi-stream framework could boost the performance further~\cite{qian2021audio}. This is because the two modalities might complement each other in situations when one of them makes a wrong decision or is absent. Based on this multi-stream framework has lately attracted more and more attention. At the 2019 NIST Speaker Recognition Evaluation challenge, it was proposed to use visual information in conjunction with the audio recordings to increase robustness of recognition frameworks~\cite{sadjadi20202019, alam2020analysis}. Apart from this, several versions of VoxCeleb - a large-scale audio-visual person recognition dataset - have been published~\cite{nagrani2017voxceleb, chung2018voxceleb2, nagrani2020voxceleb}. These datasets further boosted the development of audio-visual recognition methods~\cite{qian2021audio, chen2020multi, shon2019noise, shon2020multimodal}.





Up to date, a lot of research has been conducted on the utilization of audio or/and visual streams. In the field of speaker recognition, Chung et al. investigated multiple metric-based and softmax-based loss functions under identical conditions in order to identify which produce the best representation of an audio stream~\cite{chung2020defence}. Whereas, Yao et al. developed a new multi-stream Convolutional Neural Network which performs speaker verification tasks by a frequency selection technique - dividing the audio into different frequencies and selecting the one that describes the target best~\cite{yao2020multi}. 


In the field of person recognition, Shon et al.~\cite{shon2019noise} proposed an attention-based approach with a feature-level fusion method. The attention mechanism at the core of the network learns to select a more salient modality, which enables the model to be resistant to situations in which either of the modalities is corrupted. Their subsequent work~\cite{shon2020multimodal} introduced fine-tuning of their pre-trained unimodal models in order to prevent overfitting. Chen et al.~\cite{chen2020multi} in their end-to-end multi-modal system explored and compared three methods of fusing voice and face embeddings: Simple Soft Attention Fusion~\cite{shon2019noise}, Compact Bilinear Pooling Fusion~\cite{fukui2016multimodal}, and Gated Multi-Modal Fusion~\cite{arevalo2017gated}. In addition, the authors explored the systems with two loss functions, namely Contrastive Loss with Aggressive Sampling Strategy and Additive Angular Margin Loss~\cite{deng2019arcface}. Qian et al.~\cite{qian2021audio} proposed three audio-visual deep neural networks (AVN) for multi-modal person verification. These are - a feature level AVN (AVN-F), which accepts audio and visual streams simultaneously, an embedding-level AVN (AVN-E), which accepts pre-trained voice and face embeddings, and an embedding level AVN with joint learning (AVN-J), which optimizes unimodal models together with a fusion module resulting in an end-to-end training process. In order to evaluate the proposed AVNs on noisy data, a couple of data augmentation techniques were designed: a feature-level multi-modal data augmentation and an embedding-level noise distribution matching data augmentation. 

All of the above-mentioned works utilized two modalities, that are audio recordings and visual images. In this paper using the SpeakingFaces dataset we explore how 3 modalities — audio, visual and thermal streams — can affect the overall performance of a person verification task. 
\fi

\iffalse
Person recognition has been an active field of research for several decades~\cite{zhang2017end, snyder2018x, taigman2014deepface, wen2016discriminative}. Many approaches that have been already proposed are based on a single-stream framework, which is either on a person's voice or on his or her facial appearance, and many of them evolved over time. For example, the approaches for speaker recognition started from traditional probabilistic approaches~\cite{reynolds2000speaker, dehak2010front} and moved to deep speaker embedding ones~\cite{variani2014deep, snyder2017deep}. Whereas the approaches for face recognition have transferred from local descriptors based learning~\cite{cao2010face, lei2013learning} to deep convolutional neural networks~\cite{krizhevsky2012imagenet, parkhi2015deep, schroff2015facenet}.

Although single modality person recognition showed competitive performance, it was inferred that multi-stream framework could boost the performance further~\cite{qian2021audio}. This is because the two modalities might complement each other in situations when one of them makes a wrong decision or is absent. Based on this multi-stream framework has lately attracted more and more attention. At the 2019 NIST Speaker Recognition Evaluation challenge, it was proposed to use visual information in conjunction with the audio recordings to increase robustness of recognition frameworks~\cite{sadjadi20202019, alam2020analysis}. Apart from this, several versions of VoxCeleb - a large-scale audio-visual person recognition dataset - have been published~\cite{nagrani2017voxceleb, chung2018voxceleb2, nagrani2020voxceleb}. These datasets further boosted the development of audio-visual recognition methods~\cite{qian2021audio, chen2020multi, shon2019noise, shon2020multimodal}.
\fi

==> Odyssey 2022 Latex Template/3_dataset.tex <==
%General dataset information
In this work, we utilized the SpeakingFaces dataset~\cite{abdrakhmanova2021speakingfaces} to train, validate, and test the person verification systems.
SpeakingFaces is a publicly available multimodal dataset comprised of audio, visual, and thermal data streams.
The dataset consists of 13,711 recordings of imperative sentences\footnote{Verbal commands given to virtual assistants and other smart devices, such as `turn off the lights', `play the next song', etc.} spoken by 142 speakers from different backgrounds (i.e., around 100 utterances per speaker).
%The audio (44.1 kHz) and visual (resolution $1920\times1080$) streams were recorded using a web-camera (Logitech C920 Pro HD), while the thermal (resolution $464\times348$) stream was captured with a thermal camera (FLIR T540).
The audio and visual streams were recorded using a webcam (Logitech C920 Pro HD), while the thermal stream was captured with a high-resolution thermal camera (FLIR T540).
The data were acquired approximately one meter away from the person.
%The audios were recorded using a built-in microphone (44.1 kHz) of a web-camera (Logitech C920 Pro HD) at a distance of approximately one meter.

%Applied preprocessings
To prepare the dataset for the person verification task, we first detected bounding boxes of facial regions in visual images using RetinaFace~\cite{deng2019retinaface}.
Next, we mapped the detected bounding boxes onto the thermal images by aligning the visual and thermal streams.
Additionally, we manually filtered out from the final dataset those utterances where faces were not detected or where facial features were obscured based on previously documented artifacts.
This left 13,036 recordings in the final version.
We also downsampled the audio recordings to 16 kHz.
The samples of visual and thermal facial image pairs are shown in Figure~\ref{fig:faces} and the specifications of the preprocessed dataset are listed in Table~\ref{tab:dataset}.
%A sample recording is depicted in Figure~\ref{fig:faces} and specifications of preprocessed SpeakingFaces is given in Table~\ref{tab:dataset}. %, and the dataset can be accessed depicts a sample recordings and  here\textsuperscript{\ref{ft:github}}.

\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\columnwidth,trim={0.15cm 10.0cm 16.5cm 0.0cm},clip=true]{Figures/faces.png}
  \vspace{-0.7cm}
  \caption{The samples of visual and thermal facial image pairs in the preprocessed SpeakingFaces dataset}
  \label{fig:faces}
\end{figure}

\begin{table}[t]
\vspace{-0.2cm}
\caption{Preprocessed SpeakingFaces dataset specification}
\label{tab:dataset}
\vspace{0.2cm}
\centering
\renewcommand\arraystretch{1.1}
\setlength{\tabcolsep}{2.75mm}
    \begin{tabular}{l|c|c|c|c|c}
        \toprule
        \multicolumn{2}{l|}{\textbf{Category}}                      & \textbf{Train}& \textbf{Valid}& \textbf{Test} & \textbf{Total} \\
        \midrule
        \multicolumn{2}{l|}{\# Speakers}                            & 100           & 20            & 22            & 142 \\
        \multicolumn{2}{l|}{\# Utterances}                          & 9,307         & 1,843         & 1,886         & 13,036 \\
        \multicolumn{2}{l|}{Total duration}             & 10.4 hr       & 2.2 hr        & 2.3 hr        & 14.9 hr \\
        %\multirow{4}{*}{\scell{Utterance\\duration}}    & Total     & 10.4 hr       & 2.2 hr        & 2.3 hr        & 14.9 hr \\
                                                        %& Total     & 37557.424     & 7899.473      & 8251.730      & 53708.627 \\
                                                        %& Mean      & 4.0 s         & 4.3 s         & 4.4 s         & 4.1 s \\
                                                        %& Mean      & 4.035         & 4.286         & 4.375         & 4.12 \\
                                                        %& Min       & 1.4 s         & 1.4 s         & 2.0 s         & 1.4 s \\
                                                        %& Min       & 1.422         & 1.393         & 2.0           & 1.393 \\
                                                        %& Max       & 13.3 s        & 10.6 s        & 12.8 s        & 13.3 s \\
                                                        %& Max       & 13.332        & 10.595        & 12.831        & 13.332 \\
        \bottomrule
    \end{tabular}
\vspace{-0.3cm}
\end{table}

%Evaluation set preparation
We prepared the train, validation, and test sets following the format of VoxCeleb~\cite{nagrani2017voxceleb}.
%In particular, the train list contains the subject identifier, the file path, and one line per utterance. 
In particular, the train list contains the paths to the recordings and the corresponding subject identifiers. 
We designed \textit{easy} and \textit{hard} versions of the test and validation lists.
In the \textit{easy} version, the evaluation lists consist of randomly generated positive and negative pairs, with the numbers of pairs in the validation and test sets equal to 38,000 and 46,200, respectively.
%In total, the numbers of pairs in the validation and test sets are 38,000 and 46,200, respectively.
%There are two types of evaluation (validation and test) lists: easy and hard. In the easy case, lists consist of randomly generated positive and negative pairs. In the hard case, the randomly generated pairs are comprised of subjects with the same gender. In both cases, the same number of positive and negative pairs were selected for each subject. 
In the \textit{hard} version, the negative pairs were randomly selected from subjects belonging to the same gender, resulting in 36,400 and 44,000 pairs in the validation and test sets, respectively.
%Additionally, we generated harder evaluation lists where negative pairs were selected from the subjects belonging to the same gender. 
%The number of pairs in the harder validation and test sets are 36,400 and 44,000, respectively.
Overall, the sets are gender balanced and have similar age and race distributions.
The file structure of the prepared SpeakingFaces dataset for multimodal person verification task is shown in Figure~\ref{fig:file_struc}.

\begin{figure}[t]
    %\vspace{-0.45cm}
    \centering 
    %\tiny
    \scriptsize
    \begin{forest}
        for tree={
            font=\sffamily,
            grow'=0,
            inner sep=1.75pt,
            folder indent=0.0em,
            folder icons,
            edge=densely dotted
        }
        [SpeakingFaces, this folder size=-5pt
            [data, this folder size=8pt
                [sub\_1, this folder size=8pt
                    [rgb, this folder size=8pt
                        [\textit{subID\_trialID\_2\_posID\_commandID\_frameID\_7.png}, is file]
                        [\textbf{\dots}, is file]]
                    [thr, this folder size=8pt
                        [\textit{subID\_trialID\_2\_posID\_commandID\_frameID\_6.png}, is file]
                        [\textbf{\dots}, is file]]
                    [wav, this folder size=8pt
                        [\textit{subID\_trialID\_2\_posID\_commandID\_1.wav}, is file]
                        [\textbf{\dots}, is file]]]
                [\textbf{\dots}, this folder size=8pt]
                [sub\_142, this folder size=8pt
                    [\textbf{\dots}, is file]]]
            [metadata, this folder size=8pt
                [\textit{train\_list.txt}, is file]
                [\textit{valid\_pairs\_easy.txt}, is file]
                [\textit{test\_pairs\_easy.txt}, is file]
                [\textit{valid\_pairs\_hard.txt}, is file]
                [\textit{test\_pairs\_hard.txt}, is file]
                ]
        ]
    \end{forest}
    %\vspace{-0.25cm}
    \caption{The file structure of the SpeakingFaces dataset for the multimodal person verification task}\label{fig:file_struc}
\end{figure}

\iffalse
%Noisy version
Furthermore, to imitate more challenging scenarios, we constructed noisy version of the train and evaluation sets.
The noisy version was constructed using the Algorithm 1 of~\cite{qian2021audio}.
To distinguish the noisy version, we will append `\textit{noisy\_}' prefix.

%Missing version of eval sets
Furthermore, to imitate more challenging evaluation scenarios, we constructed additional two versions of the evaluation sets: 1) missing and 2) noisy.
The former imitates the failure of some modality, which was implemented by setting values of the missing modality in the evaluation set to zero.
%We tried two approaches; setting the values of missing modality in the validation and test sets to (1) zero and (2) random number.
To distinguish this version from others, we will append \textit{missA}, \textit{missV}, and \textit{missT} prefixes which indicate the failure of audio, visual, and thermal streams, respectively.
Likewise, the failure of audio and visual streams will be indicated using \textit{missAV} prefix.
\fi

%Noisy version of eval sets
%Furthermore, 
To imitate more challenging scenarios, we deployed a noisy version of the train, validation, and test sets.
The noisy data were constructed using Algorithm 1 presented in~\cite{qian2021audio}.
%To construct the noisy evaluation set, we followed the Algorithm 1 presented in~\cite{nagrani2017voxceleb}.
In particular, for the visual stream, we applied vertical and horizontal motion blur, to imitate the motion of a person in front of the camera, and the Gaussian blur, to imitate other noises.
For the thermal stream, we applied only the Gaussian blur.
For the audio stream, we added three kinds of noises from the Musan dataset~\cite{DBLP:journals/corr/SnyderCP15}. % with \textbf{0 dB SNR}.
In addition, for all streams, we used random noise sampled from the standard normal distribution (i.e., $\mathcal{N}(0,1)$) to imitate a broken data stream.
%To distinguish the noisy version, we will append `\textit{noisy\_}' prefix.
%The noisy versions of evaluation sets will be prepended with the \textit{noisyA}, \textit{noisyV}, and \textit{noisyT} prefixes indicating the presence of aforementioned noises in audio, video, and thermal streams.
%The \textit{noisyALL} prefix will be used to indicate the presence of noise in all streams.
%The final version of the preprocessed SpeakingFaces can be accessed here\footnote{\url{link_to_dataset}}.

%This dataset opens up interesting opportunities for the future research and has the potential to facilitate a diverse set of ongoing research in multi-modal learning, such as (visual-thermal) lip reading, (audio-visual-thermal) speech, gender, and age recognition, and so on.

%
%\begin{figure}[t]
%\includegraphics[width=\columnwidth]{paper_completion.pdf}
%\caption{{\it This is an example of a figure.}}
%\label{spprod}
%\end{figure}
%


\iffalse
\begin{figure}[tb]
  \centering
    \includegraphics[width=1.0\linewidth,trim={0.0cm 9.15cm 20.5cm 0.0cm},clip=true]{Figures/sample.png}
%    \vspace{2.0cm}
    \caption{A sample recording snapshots taken every 0.5 seconds of a speaker uttering `stop the kitchen fan from turning'.}
    \label{fig:faces}
\end{figure}

\begin{table}[th]
\caption{\label{table1} {\it This is an example of a table.}}
\vspace{2mm}
\centerline{
\begin{tabular}{|c|c|}
\hline
ratio & decibels \\
\hline  \hline
1/1 & 0 \\
2/1 & $\approx$ 6 \\
3.16 & 10 \\
10/1 & 20 \\
1/10 & -20 \\
100/1 & 40 \\
1000/1 & 60 \\
\hline
\end{tabular}}
\end{table}
\fi




%For the purpose of this research we used all frames. The first step into data preprocessing was to detect faces. The detection was done with the help of RetinaFace proposed by \url{https://github.com/deepinsight/insightface/tree/master/detection/RetinaFace}. RetinaFace was incorporated in \url{https://github.com/IS2AI/SpeakingFaces/blob/master/build_face_img_data.py}. 

%The frames that were undetected by RetinaFace were collected in \textit{log.txt} file. Other than \textit{log.txt} coming from RetinaFace, we had \textit{log.dnn.txt}, which is all frames that DNN model could not detect. Our aim was to clean the dataset as much as possible such that it will be free from different artifacts that are too terrible, and for that we had to manually check some of the utterances that seem to be suspicious.\\
%In order to understand which utterances are worth re-checking, we referred to our \textit{log.dnn.txt}, \textit{log.txt} and csv files containing the information about the artifacts. We firstly removed all utterances belonging to \textit{log.txt} from the \textit{log.dnn.txt}, and also removed those utterances that did not have any artifacts. There were in total 70 utterances we had to check manually and decide which of them are acceptable and which of them should be removed for our purposes. Since each utterance contained 150 frames (images) on average, in order to accelerate the process of the manual check, we have decided to collect them together and make videos for each utterance. After some manipulations, from the \textit{log.dnn.txt} file we had 70 videos to check. We were checking both rgb and thr streams. \\
%Our rejection criteria, in the case of rgb stream, were either the frames are terribly blurry, or the chin is cropped (because of alignment), and for the thr stream, it was the frames were frozen for some time.\\
%There were also other lists of potential utterances that are problematic, namely \textit{black.list.false.txt}, \textit{black.list.blurry.txt}, \textit{black.list.cropped.txt} which were collected by manual observations. We also took a look at these utterances and have decided which to accept or reject based on the above criteria. Apart from that, since validation and test sets are very important for the evaluation, it was crucial to check all these utterances as well. \\
%We created a large csv which was a collection of all 142 csv files containing the information about the artifacts, we also added two new columns indicating subject id and trial id. \\
%After systematically deciding which utterances to delete and which to accept, we dropped all the utterances that were rejected from the giant csv, and also dropped those belonging to \textit{log.txt}, the ones that RetinaFace could not detect. \\

%There were 13711 utterances in the beginning, and after some check-ups and cleaning the number of utterances was reduced to 13589 utterances. However since some of them contained no transcription, we needed to drop such cases too ending up with 13042 utterances in total. We dropped 6 more utterances that did not have audio-files, so the final dataset now has 13036 utterances in total.\\
%In the end, in order to make our dataset in the proper format such that it would fit to our model, we redistributed all the data by folders.


==> Odyssey 2022 Latex Template/4_method.tex <==
We followed~\cite{chung2020defence} to implement the multimodal person verification system. 
The system architecture is depicted in Figure~\ref{fig:arch} which consists of two main modules: encoder and fusion.
The encoder module is responsible for extracting high-level feature representations from different modalities, and the fusion module is used to combine the extracted features.

\begin{figure}[thb]
  \centering
  \includegraphics[width=0.65\columnwidth,trim={0.0cm 8.75cm 22.5cm 0.0cm},clip=true]{Figures/architecture2.png}
%    \vspace{2.0cm}
  \caption{The audio-visual-thermal person verification network architecture}
  \label{fig:arch}
\end{figure}

\subsection{Encoder module}
The encoder module $Encoder(\cdot)$ is based on the ResNet34~\cite{DBLP:conf/cvpr/HeZRS16} network.
%Specifically, for images (i.e., visual and thermal), we used the original ResNet34 network with the halved number of channels in each residual block to reduce computational cost.
Specifically, for image input (i.e., visual and thermal), we used a variation of ResNet34, in which the number of channels in each residual block is halved in order to reduce computational costs.
For audio, we used another variation of ResNet34, in which average-pooling was replaced with self-attentive pooling (SAP)~\cite{DBLP:conf/odyssey/CaiCL18} to aggregate frame-level features into an utterance-level representation.
%except with only half of the channels in each residual block in order to reduce computational cost.

The encoder takes in a raw feature $x_{i}$ and outputs the corresponding embedding vector representation $e_{i}\in\mathbb{R}^{512}$:
\begin{equation}
e_{i} = Encoder(x_{i})
\end{equation}
where $i\in\{a,v,t\}$ is used to represent the stream source (i.e., audio, visual, and thermal).
We trained a separate encoder module for each data stream.

\subsection{Fusion module}
%As a fusion module, we tried two different approaches: 1)~embedding-level and 2)~score-level.
%In the embedding-level fusion, we implemented a soft attention mechanism similar to that in~\cite{shon2019noise}, where the fusion module can pay attention to a salient modality among audio $e_a$, visual $e_v$, and thermal $e_t$ representations.
As a fusion module, we tried two different approaches: 1)~attention mechanism and 2)~score averaging.

\subsubsection{Attention mechanism}
In the attention-based approach, we implemented an embedding-level fusion similar to that in~\cite{shon2019noise}, where the fusion module can pay attention to a salient modality among audio $e_a$, visual $e_v$, and thermal $e_t$ representations.
Specifically, it first computes the attention score $\hat{\alpha}_{\{a,v,t\}}\in \mathbb{R}^3$ as follows:
\begin{equation}
\hat{\alpha}_{\{a,v,t\}} = \mathbf{W}[e_a,e_v,e_t]+\mathbf{b}
\end{equation}
where the weight matrix $\mathbf{W}\in\mathbb{R}^{3\times1536}$ and the bias vector $\mathbf{b}\in\mathbb{R}^3$ are learnable parameters.
%The $e_a$, $e_v$, and $e_t$ are embedding vectors produced by the encoder module corresponding to audio, video, and thermal streams, respectively.
%Next, the attention scores are normalized and the fused person embedding vector $e_p$ is produced by the weighted sum:
Next, the fused person embedding vector $e_p$ is produced by the weighted sum:
\begin{equation}
e_p=\sum_{i\in\{a,v,t\}}\alpha_ie_i\text{\ \ , where\ \ } \alpha_i=\frac{\exp(\hat{\alpha}_i)}{\sum_{k\in\{a,v,t\}}\exp(\hat{\alpha}_k)}
\end{equation}
%The embedding-level fusion for the audio-visual bimodal systems was designed in a similar manner, where two modalities are used instead of three.
The attention-based fusion for the bimodal systems (i.e., audio-visual) was designed in a similar manner, using two modalities instead of three.
Note that the attention-based fusion module is jointly trained with the encoder modules in an end-to-end fashion.
%Lastly, the fused person embedding vector $e_p$ is produced by the weighted sum:
%\begin{equation}
%e_p=\sum_{i\in\{a,v,t\}}\alpha_ie_i
%\end{equation}

\subsubsection{Score averaging}
%In the score-level fusion, we simply averaged the scores $s_i\in[0,2]$ produced by the unimodal verification systems, where a score is the Euclidean distance between two test subjects as will be described in the following section.
In the score-level fusion, we simply averaged the scores $s_i\in[0,2]$ produced by the unimodal verification systems, where a score is the Euclidean distance between two normalized speaker embeddings.
For example, for the trimodal system, the final score $s_{\textit{final}}$ is computed as follows:
\begin{equation}
s_{\textit{final}} = \frac{\sum_{i\in\{a,v,t\}}s_i}{3}
\end{equation}
Likewise, for the bimodal system, the final score is computed by averaging the scores of two unimodal systems. 

==> Odyssey 2022 Latex Template/5_exp_setup.tex <==
All the person verification models were trained on a single V100 GPU running on the NVIDIA DGX-2 server using the training set.
%Specifically, the overall network architecture was jointly optimized in an end-to-end fashion.
All hyper-parameters were tuned using the validation set, and the settings for each modality were tuned separately.
The best performing model on the validation set was evaluated using the test set.
%Note that these experiments are intended as an initial exploration into audio-visual-thermal person verification, therefore, the extensive hyper-parameter tuning, detailed analyses of various loss functions, and other sophisticated methods were left for future work.
%To generate the noisy versions of data, we set the noise rate in Algorithm 1 to 30\%.

At the training stage, input features from the audio stream were generated by randomly extracting a two-second segment from each recording and then transforming it into 40-dimensional mel spectogram features.
For the visual and thermal streams, we extracted the first frame of a recording. %, and then \textbf{mean normalized} the frame.
%The extracted frames were mean normalized and zero-centered.
Model parameters were optimized using the angular prototypical~\cite{chung2020defence} loss function. % and AAM-Softmax [cite] loss functions.
Each batch contained all the 100 speakers of the train set with nine utterances per speaker.
%For angular prototypical loss, bla-bla (initial learning rate, batch construction, lr reduction, and etc.).
%For AAM-Softmax, bla-bla.
%We set the batch size to X with the equal number of positive and negative pairs.
%The [cite] with the initial learning rate of X for X epochs.
%The learning rate decreased by X\% every X epochs.
As a regularization, we applied weight decay tuned for each model separately.
%The best-performing model on the validation set was evaluated using the clean and noisy versions of the test set.
%The system implementation including the model specifications and other hyper-parameter values are provided in our GitHub repository\footnote{\url{GitHub_link}}.
We trained each model three times with a different seed number and report the mean and standard deviation of the results.
The exact system implementation details are provided in our GitHub repository\textsuperscript{\ref{ft:github}}.

At the evaluation stage, from each test recording, we extracted ten two-second audio segments at regular intervals, and ten equidistantly spaced image frames.
%, and then \textbf{mean normalized} the frames.
%In the unimodal setting, we computed a similarity score between all possible combinations (10×10 = 100) from every pair.
In the multimodal setting with attention, for a given utterance, each of the ten audio segments was paired with an image frame from either or both modalities.
%Similarly to the unimodal settting, 
We computed a similarity score between all possible combinations (10×10 = 100) from each pair of utterances present in the evaluation sets.
As a similarity score, we used the Euclidean distance, and the mean of the 100 similarities was used as the final score.
The performance of the models was evaluated using the EER metric. 
%The performance of models was measured using both Equal Error Rate (EER) and minimum Detection Cost Function (minDCF) ($P_{target} = 0.01$)~\cite{sadjadi20172016}. 


%The noisy versions of train and evaluation sets were generated using 30\% noise rate.

==> Odyssey 2022 Latex Template/6_exp_results.tex <==
\begin{table*}[htb]
\caption{EER (\%) performance results (mean $\pm$ std) of person verification systems on the \textit{easy} evaluation set under two conditions:\\1) \textit{clean} and 2) \textit{noisy}. Under the \textit{noisy} condition, the percentages of noisy samples in the train, validation, and test sets were set to 30\%.}
\label{tab:results}
\vspace{2mm}
\centering
\renewcommand\arraystretch{1.1}
\setlength{\tabcolsep}{3.5mm}
    \begin{tabular}{l|c|cc|cc}
        \toprule
        \multirow{2}{*}{\textbf{Modality}}  & \multirow{2}{*}{\textbf{Fusion}}  &   \multicolumn{2}{c|}{\textit{\textbf{clean}}}             & \multicolumn{2}{c}{\textit{\textbf{noisy}}} \\\cline{3-6}
                                        &                           &  \textbf{valid}           & \textbf{test}         & \textbf{valid}    & \textbf{test} \\
        \midrule
        Audio                           & -                         & $10.82\pm0.39$            & $9.29\pm0.15$         & $15.03\pm0.54$    & $11.86\pm0.30$ \\
        Visual                          & -                         & $4.04\pm0.89$             & $4.09\pm0.86$         & $5.81\pm0.67$     & $4.36\pm0.93$ \\
        Thermal                         & -                         & $10.30\pm0.74$            & $10.58\pm1.28$        & $11.00\pm1.18$    & $12.72\pm0.93$ \\\hline
        \multirow{2}{*}{Audio-Visual}   & Attention                 & $4.42\pm0.85$             & $3.69\pm0.44$         & $5.46\pm1.01$     & $4.10\pm1.07$ \\.  
                                        & Score averaging           & $2.39\pm0.42$             & $2.20\pm0.58$         & $3.69\pm0.48$     & $2.61\pm0.45$ \\\cline{1-6}
        \multirow{2}{*}{Audio-Visual-Thermal}       & Attention                 & $3.44\pm0.60$             & $2.90\pm0.15$         & $4.02\pm1.02$     & $3.74\pm1.04$ \\
                                        & Score averaging           & \textbf{2.26 $\pm$ 0.10}  & \textbf{1.80 $\pm$ 0.31} & \textbf{2.92 $\pm$ 0.22} & \textbf{2.13 $\pm$ 0.47} \\
        \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[htb]
\caption{EER (\%) performance results (mean $\pm$ std) of person verification systems on the \textit{hard} evaluation set under two conditions:\\1) \textit{clean} and 2) \textit{noisy}. Under the \textit{noisy} condition, the percentages of noisy samples in the train, validation, and test sets were set to 30\%.}
\label{tab:results_samegender}
\vspace{2mm}
\centering
\renewcommand\arraystretch{1.1}
\setlength{\tabcolsep}{3.5mm}
    \begin{tabular}{l|c|cc|cc}
        \toprule
        \multirow{2}{*}{\textbf{Modality}}  & \multirow{2}{*}{\textbf{Fusion}}  &   \multicolumn{2}{c|}{\textit{\textbf{clean}}}             & \multicolumn{2}{c}{\textit{\textbf{noisy}}} \\\cline{3-6}
                                        &                           &  \textbf{valid}           & \textbf{test}         & \textbf{valid}    & \textbf{test} \\
        \midrule
        Audio                           & -                         & $15.14\pm0.27$            & $14.13\pm0.12$         & $21.34\pm0.88$    & $17.99\pm1.01$ \\
        Visual                          & -                         & $5.60\pm0.91$             & $5.23\pm0.68$         & $6.85\pm0.86$     & $5.84\pm1.58$ \\
        Thermal                         & -                         & $13.21\pm1.07$            & $12.34\pm1.28$        & $13.25\pm1.32$    & $14.81\pm2.33$ \\\hline
        \multirow{2}{*}{Audio-Visual}   & Attention                 & $5.72\pm0.98$             & $4.89\pm0.42$         & $6.71\pm1.15$     & $5.61\pm1.61$ \\
                                        & Score averaging           & $3.48\pm0.64$             & $3.10\pm0.42$         & $5.33\pm0.43$     & $3.89\pm0.58$ \\\cline{1-6}
        \multirow{2}{*}{Audio-Visual-Thermal}       & Attention                 & $4.40\pm0.83$             & $4.72\pm1.49$         & $5.18\pm1.26$     & $5.18\pm1.73$ \\
                                        & Score averaging           & \textbf{3.07 $\pm$ 0.55}  & \textbf{2.53 $\pm$ 0.38} & \textbf{3.96 $\pm$ 0.12} & \textbf{3.40 $\pm$ 0.78} \\
        \bottomrule
\end{tabular}
\end{table*}

We evaluated the performance of unimodal and multimodal person verification systems on \textit{easy} and \textit{hard} evaluation lists under 
%three different conditions: 1) \textit{train clean / evaluation (i.e., validation and test sets) clean}, 2) \textit{train clean / evaluation noisy}, and 3) \textit{train noisy / evaluation noisy}.
two data conditions: 1) \textit{clean} and 2) \textit{noisy}.
The noisy versions of the train, validation, and test sets were generated based on the procedure described in Section~\ref{sec:dataset}.
%The evaluation lists that consist of the same gender negative pairs are denoted as \textit{hard}, while the evaluation lists with no such constraint are labeled as \textit{easy}.

\begin{figure}[b]
    \centering
    \includegraphics[width=0.5\columnwidth,clip=true]{Figures/venn_diag_err3.png}
%    \vspace{2.0cm}
    \caption{The verification error statistics of unimodal systems}
    \label{fig:ver_errors}
\end{figure}

\subsection{Unimodal Person Verification}
%We first conducted the unimodal person verification experiments under the three different conditions:
%1) \textit{train clean / evaluation (i.e., validation and test sets) clean}, 2) \textit{train clean / evaluation noisy}, and 3) \textit{train noisy / evaluation noisy}.
%The noisy versions of the train and evaluation sets were generated based on the process described in Section~\ref{sec:dataset}, where the noise rate was set to 30\%.
The results of the unimodal person verification experiment on the \textit{easy} test set are given in the first part of Table~\ref{tab:results}.
When train and evaluation sets are clean, the best EER performance is achieved by the visual modality (4.09\%), followed by the audio modality (9.29\%) and then the thermal modality (10.58\%).
Under the noisy condition, the performance degrades by 28\%, 7\%, and 20\% relative EER for the audio, visual, and thermal systems, respectively.
According to these results, the visual system performs the best and is more robust to corrupted data.

Interestingly, the results in Table~\ref{tab:results_samegender} show that the best EER performance on the \textit{hard} test set, under the clean condition, is achieved by the visual modality (5.23\%), followed by the thermal modality (12.34\%) and then the audio modality (14.13\%).
%These results indicate that thermal modality has higher same gender discrimination power\footnote{At least in our experiment settings.}.
%These results indicate that thermal modality surpasses audio on the same gender verification task\footnote{At least in our experiment settings.}.
%These results indicate that thermal modality is better than audio on the same gender discrimination\footnote{At least in our experiment settings.}.
%These results indicate that thermal modality is better than audio on differentiating the same gender pairs\footnote{At least in our experiment settings.}.
%These results indicate that thermal modality possess higher discriminate power for the same gender verification task.
Under the noisy condition, the performance degrades by 27\%, 12\%, and 20\% relative EER for the audio, visual, and thermal systems, respectively.
These results indicate that the visual system remains superior, but the thermal modality outperforms the audio in differentiating subjects of the same gender\footnote{At least in our experimental settings.}.
%In the second condition, where evaluation sets are noisy, the EER performances on the test set deteriorate by 60\%-82\% relative to the first condition.
%Presumably, this is due to the domain mismatch between train and evaluation sets.
%In the noisy condition, the EER performances on the test set degrades by 7\%-27\% relative to the clean condition.
%This result demonstrates that training data augmentation is effective on reducing the negative effects of the noisy data.

%To further examine the performance of unimodal systems, we computed accuracy on the \textit{easy} test set under the \textit{clean} condition, separating the pairs with same and opposite gender.
To further examine the performance of the unimodal systems, we computed accuracy on the \textit{easy} test set under the \textit{clean} condition, separating the same- and opposite-gender pairs.
The results are presented in the first part of Table~\ref{tab:results_acc}.
Following the observations from the above, when a given pair of subjects belong to the same gender, the visual modality (95.07\%) is superior, while the thermal modality (88.06\%) is better than the audio modality (86.72\%). 
However, the audio modality (98.45\%) performs the best in distinguishing subjects of opposite gender.
%deciding between subjects of the same gender compared to 
\iffalse
The results show that the EER performances of unimodal models on the test set deteriorate under the second condition by 60\%-82\% relative to the first condition.
Presumably, this is due to the domain mismatch between train and evaluation sets.
In the third condition, where the noise rates in the train and evaluation sets are matched, the EER performances on the test set degrades by 7\%-27\% relative to the first condition.
These results demonstrate the poor robustness of unimodal systems under the noisy conditions.
Overall, the best EER is achieved by visual modality followed by audio and then thermal in all three conditions.
\fi

We also analysed the verification errors made by the unimodal systems on the \textit{easy} test set under the \textit{clean} condition (see Figure~\ref{fig:ver_errors}).
We observed that the number of overlapping errors between different modalities is lower than the errors made by a single modality.
%We observed that the overlapped errors between different modalities are fewer than the errors made by a single modality.
This indicates that these modalities posses strong complementary properties, and therefore, multimodal systems that can combine them effectively have good potential. 
Future work should focus on analysing these errors in great detail to identify the weaknesses and strengths of each modality.

\iffalse
\begin{table}[h]
\centering
%\renewcommand\arraystretch{1.1}
%\setlength{\tabcolsep}{1.1mm}
    \begin{tabular}{l|c|c}
        \toprule
        \multirow{2}{*}{Modality}           & \multicolumn{2}{c}{EER (\%)} \\\cline{2-3}
                                            & Valid     & Test \\ 
        \midrule
        Visual                              &           & \\
        Audio                               &           & \\
        Thermal                             &           & \\

        \bottomrule
\end{tabular}
\caption{Unimodal person verification results.}
\label{tab:uni}
\end{table}
\fi 

\begin{table}[t]
%\small	
\caption{Accuracy (\%) results (mean $\pm$ std) on the \textit{easy} test set. The data condition is \textit{clean} and multimodal systems are based on score fusion. Bimodal: Audio-Visual. Trimodal: Audio-Visual-Thermal.}
\label{tab:results_acc}
\vspace{2mm}
\centering
\renewcommand\arraystretch{1.1}
%\setlength{\tabcolsep}{1.0mm}
    \begin{tabular}{l|cc|c}
        \toprule
        \textbf{Modality}       & \textbf{\scell{Same\\gender}} & \textbf{\scell{Opposite\\gender}} & \textbf{Overall}\\
        \midrule
        Audio                   &   $86.72\pm1.88$              & $98.45\pm1.35$                    & $89.79\pm1.73$\\
        Visual                  &   $95.07\pm0.86$              & $98.28\pm0.90$                    & $95.91\pm0.87$\\
        Thermal                 &   $88.06\pm1.75$              & $93.24\pm0.70$                    & $89.41\pm1.29$\\\hline
        Bimodal                 &   $97.07\pm0.73$              & $99.87\pm0.17$                    & $97.80\pm0.58$\\\hline
        Trimodal                &   \textbf{97.61 $\pm$ 0.39}   & \textbf{99.87 $\pm$ 0.08}         & \textbf{98.20} $\pm$ \textbf{0.31}\\
        \bottomrule
\end{tabular}
\end{table}


\subsection{Multimodal Person Verification}
%The multimodal person verification experiment results are given in the second part of the Table~\ref{tab:results}.
%Particularly, we built bimodal (audio-visual) and trimodal (audio-visual-thermal) verification models.

The experimental results for our bimodal (audio-visual) and trimodal (audio-visual-thermal) verification models are presented in the second and third parts of Table~\ref{tab:results} and Table~\ref{tab:results_samegender}, respectively.
%We constructed these models using two fusion methods, the soft attention and the score averaging, as mentioned in the previous sections.
The models were constructed using two fusion methods, soft attention and score averaging, as mentioned in the previous sections.
%To construct these models, we used two different fusion approaches based on the soft attention and the score averaging, as  mentioned in the previous sections.
The latter approach provides superior performance for both bimodal and trimodal verification systems, which is consistent with the observations made in~\cite{qian2021audio}, but different from the findings in~\cite{shon2019noise}.
%We found that the score averaging based fusion performs better than the attention for both bimodal and trimodal verification systems.
%This complies with the observations made in~\cite{qian2021audio}, but differs from the findings in~\cite{shon2019noise}.

The experimental results show that the multimodal systems outperform the unimodal systems. 
%The best bimodal system achieved 46\% (from 4.09 to 2.20) and 39\% (from 4.38 to 2.65) relative EER reductions on the test set over the visual system under the clean and noisy conditions, respectively.
For the \textit{easy} test set, the best bimodal system reduced EER by 46\% (from 4.09 to 2.20) and 40\% (from 4.36 to 2.61) relative to the visual system under the clean and noisy conditions, respectively.
The best trimodal system reduced EER by 56\% (from 4.09 to 1.80) and 51\% (from 4.36 to 2.13) under the clean and noisy conditions, respectively.
%Similarly, the best trimodal system achieved 55\% (from 4.09 to 1.80) and 51\% (from 4.38 to 2.13) relative EER reductions on the test set over the visual system under the clean and noisy conditions, respectively.
Remarkably, these improvements were achieved by simply averaging the scores of the unimodal systems.

For the \textit{hard} test set, we observed similar behaviour. The best bimodal system reduced EER by 41\% (from 5.23 to 3.10) and 33\% (from 5.84 to 3.89) relative to the visual system under the clean and noisy conditions, respectively.
The best trimodal system reduced EER by 52\% (from 5.23 to 2.53) and 42\% (from 5.84 to 3.40) under the clean and noisy conditions, respectively.
%These results demonstrate the superiority of multimodal systems over unimodal counterparts.

%Comparing the bimodal and trimodal systems, we found the trimodal system to perform better in both clean and noisy conditions, with the 18\% (from 2.20 to 1.80) and 19\% (from 2.65 to 2.13) relative EER improvements on the test set.
The trimodal system achieved better results than the bimodal system on both evaluation sets under the clean and noisy conditions.
On the \textit{easy} test set, EERs were improved by 18\% relative for both conditions (from 2.20 to 1.80, and from 2.61 to 2.13).
On the \textit{hard} test set, the trimodal system surpassed the bimodal system by 18\% (from 3.10 to 2.53) and 13\% (from 3.84 to 3.40) relative EERs, under the \textit{clean} and \textit{noisy} conditions respectively.
%Interestingly, the attention-based trimodal verification system achieved better EER  under the noisy condition (4.17 versus 3.65). 

The analysis of the attention network parameters suggests that the mechanism learned to prioritize the visual stream when the streams were not corrupted.
In contrast, the network focused on all the three streams when the data were noisy. 
%After analysing the attention network parameters, we presume that under the clean condition the attention learns to focus more on the visual stream.
%On the other hand, under the noisy condition, the attention learns to focus on all three streams.
Therefore, augmenting the train set with noise plays an important role in learning more robust features, and future work should study different augmentation methods for the multimodal person verification task.
Unfortunately, combining three modalities using the soft attention mechanism is challenging due to the instability of the training process, and further studies should be conducted to explore other attention methods.
%Overall, the results highlight that supplementing the audio-visual modalities with the thermal images enhances the EER performance of person verification systems.
%The same trends are observed in the results on the \textit{hard} evaluation sets.
Overall, the results suggest that the addition of thermal image data does indeed enhance the EER performance of multimodal person verification systems.

%These results demonstrate the effectiveness of thermal modality for the audio-visual person verification systems.
%These results demonstrate the complementary nature of thermal and audio-visual modalities.

%We observed that the combination of three modalities is challenging, because the training process is sometimes unstable.
%Therefore, the future work should focus on investigating better fusion strategies. 
%(Should we try curriculum learning - In defence of metric learning for speaker recognition).

%The combination of attention based fusion with the conventional score fusion yields further improvement, achieving the best EER and mDCF scores.
%This result demonstrates the complementary nature of two person verification approaches, which complies with the findings in~\cite{qian2021audio}.

%To highlight the importance of supplementing the audio-visual modalities with the thermal images, we computed accuracy on the same and different gender pairs of the easy test set.
The importance of supplementing the audio-visual modalities with the thermal images is also accentuated in Table~\ref{tab:results_acc}.
%The bimodal system is able to take the best of the two streams and drastically boost the accuracy results in both same and opposite gender pairs.
The bimodal system is able to take the best of the two streams and drastically boost the performance in handling both same- and opposite-gender pairs.
The addition of the thermal stream strengthens the performance of the multimodal system even further for the same gender pairs, but has an insignificant effect on the opposite gender pairs. 

%Although the bimodal system is able to take the best of the two streams and drastically boost the accuracy results in both cases (from 86.72\% and 95.07\% to 97.07\% for the same gender pairs, and from 98.45\% and 98.28\% to 99.87\% for the opposite gender pairs), the addition of thermal stream strengthens the performance of the multimodal system even further (from 97.07\% to 97.61\%). 








\iffalse
\begin{table*}[htb]
\centering
%\renewcommand\arraystretch{1.1}
%\setlength{\tabcolsep}{1.1mm}
    \begin{tabular}{l|c|cc|cc|cc}
        \toprule
        \multirow{2}{*}{Modality}       & \multirow{2}{*}{Fusion}   &   \multicolumn{2}{c|}{\scell{Train clean /\\evaluation clean}}& \multicolumn{2}{c|}{\scell{Train clean /\\evaluation noisy}}             & \multicolumn{2}{c}{\scell{Train noisy /\\evaluation noisy}} \\\cline{3-8}
                                        &                           &  valid                        & test                          & valid             & test                     & valid                     & test                    \\ 
        \midrule
        Audio                           & -                         & $10.82\pm0.39$                & $9.29\pm0.15$                 & $18.04\pm0.26$    & $16.71\pm0.41$                                           & $14.89\pm0.60$            & $11.83\pm0.62$ \\
        %Audio                               & -                         & $10.8176\pm0.3911$  & $9.2944\pm0.1498$   & $18.0386\pm0.2579$     & $16.7056\pm0.4095$  &$12.7561\pm0.5744$   &$9.54820\pm0.3790$    &$14.8895\pm0.6035$   &$11.8312\pm0.6236$   \\
        Visual                          & -                         & $4.04\pm0.89$                 & $4.09\pm0.86$                 & $6.90\pm1.44$     & $6.56\pm1.63$                                            & $5.32\pm0.63$             & $4.38\pm0.29$ \\
        %Visual                              & -                         & $4.0439\pm0.8883$     & $4.0923\pm0.8648$   &$6.9070\pm1.4377$    & $6.5613\pm1.6331$   &$5.7632\pm0.5299$    &$4.2078\pm0.0697$      &$5.3211\pm0.6328$    &$4.3766\pm0.2896$   \\
        Thermal                         & -                         & $10.30\pm0.74$                & $10.58\pm1.28$                & $19.14\pm2.52$    & $19.28\pm2.46$                                           & $11.06\pm0.20$            & $12.39\pm1.06$ \\
        %Thermal                             & -                         & $10.2982\pm0.7390$  & $10.5844\pm1.2848$  &$19.1351\pm2.5188$   & $19.2785\pm2.4635$  &$10.9877\pm1.1452$     &$12.6883\pm0.9425$   &$11.0579\pm0.1974$   &$12.3867\pm1.0605$   \\
        \midrule
        Bimodal                         & \multirow{2}{*}{Attention}& $4.42\pm0.85$                 & $3.69\pm0.44$                 & $6.51\pm0.48$     & $5.48\pm0.25$                                            & $5.03\pm0.95$             & $4.05\pm0.61$ \\
        %Bimodal                        & \multirow{2}{*}{Attention}     &$4.4245\pm0.8536$.   &$3.6854\pm0.4439$    &$6.5105\pm0.4781$    &$5.4820\pm0.2519$    &$4.9912\pm0.9701$        &$3.9625\pm0.5937$   &$5.0333\pm0.9539$        &$4.0534\pm0.6088$   \\
        Trimodal                        &                           & $4.28\pm0.38$                 & $4.17\pm1.19$                 & $5.85\pm0.82$     & $5.47\pm1.46$                                            & $4.07\pm1.03$             & $3.65\pm1.06$ \\\hline
        %Trimodal                &                                       &$4.2772\pm0.3825$.   &$4.1689\pm1.1906$    &$5.8456\pm0.8186$    &$5.4675\pm1.4585$    &$3.9439\pm1.1156$    &$3.5859\pm0.9777$      &$4.0666\pm1.0344$      &$3.6522\pm1.0619$   \\\hline
        Bimodal                         & \multirow{2}{*}{ScoreAve} & $2.39\pm0.42$                 & $2.20\pm0.58$                 & $5.45\pm0.89$     & \textbf{4.50 $\pm$ 1.05}                             & $3.70\pm0.35$             & $2.65\pm0.34$ \\
        %Bimodal                        & \multirow{2}{*}{ScoreAve}      & $2.3948\pm0.2602$       & $2.2049\pm0.2116$       & $5.4509\pm0.7323$       &$4.4993\pm0.5550$       &$3.7035\pm0.1160$       &$2.9807\pm0.1980$       &$3.7035\pm0.1160$       & $2.9807\pm0.1980$   \\
        Trimodal                        &                           & \textbf{2.26 $\pm$ 0.10}      & \textbf{1.80 $\pm$ 0.31}      & \textbf{5.31 $\pm$ 0.86}  & $4.52\pm0.59$                           & \textbf{2.98 $\pm$ 0.20}  & \textbf{2.13 $\pm$ 0.51} \\
        %Trimodal                &                                       &$2.2561\pm0.0603$       &$1.7980/pm0.1039$       & $5.3070\pm0.8440$       &$4.5195\pm0.5486$       &$2.6479\pm0.2149$       &$2.1284\pm0.3475$       & $2.6479\pm0.2149$       & $2.1284\pm0.3475$   \\
        \bottomrule
\end{tabular}
\caption{EER (\%) performance results of person verification systems under three conditions. \textit{Bimodal} and \textit{Trimodal} correspond to \textit{Audio-Visual} and \textit{Audio-Visual-Thermal} models respectively. The noise rate in both train and evaluation sets is 30\%.}
\label{tab:results}
\end{table*}


\begin{table}[h]
\centering
%\renewcommand\arraystretch{1.1}
%\setlength{\tabcolsep}{1.1mm}
    \begin{tabular}{l|c|c}
        \toprule
        \multirow{2}{*}{Modality}           & \multicolumn{2}{c}{EER (\%)} \\\cline{2-3}
                                            & Valid     & Test \\ 
        \midrule
        Audio-Visual                        &           & \\
        Audio-Visual-Thermal                &           & \\
        \bottomrule
\end{tabular}
\caption{Multi-modal person verification results.}
\label{tab:multi}
\end{table}


\begin{table*}[t]
\centering
%\renewcommand\arraystretch{1.1}
%\setlength{\tabcolsep}{1.1mm}
    \begin{tabular}{l|c|cc|cc|cc|cc}
        \toprule
        \multirow{2}{*}{Modality}           & \multirow{2}{*}{Fusion}   &   \multicolumn{4}{c|}{Train clean}   & \multicolumn{4}{c}{Train noisy} \\\cline{3-10}
                                            &                           & valid & test & valid' & test' & valid & test & valid' & test' \\ 
        \midrule
        Audio                               & -                         & $10.8\pm0.4$  & $9.3\pm0.2$   &$18\pm0.3$     & $16.7\pm0.4$  &$12.8\pm0.6$   &$9.5\pm0.4$    &$14.9\pm0.6$   &$11.8\pm0.6$   \\
        %Audio                               & -                         & $10.8176\pm0.3911$  & $9.2944\pm0.1498$   &$18.0386\pm0.2579$     & $16.7056\pm0.4095$  &$12.7561\pm0.5744$   &$9.54820\pm0.3790$    &$14.8895\pm0.6035$   &$11.8312\pm0.6236$   \\
        Visual                              & -                         & $4\pm0.9$     & $4.1\pm0.9$   &$6.9\pm1.4$    & $6.5\pm1.6$   &$5.8\pm0.5$    &$4.2\pm1$      &$5.3\pm0.6$    &$4.4\pm0.3$   \\
        %Visual                              & -                         & $4.0439\pm0.8883$     & $4.0923\pm0.8648$   &$6.9070\pm1.4377$    & $6.5613\pm1.6331$   &$5.7632\pm0.5299$    &$4.2078\pm0.0697$      &$5.3211\pm0.6328$    &$4.3766\pm0.2896$   \\
        Thermal                             & -                         & $10.3\pm0.7$  & $10.6\pm1.3$  &$19.1\pm2.5$   & $19.3\pm2.5$  &$11\pm1.1$     &$12.7\pm0.9$   &$11.1\pm0.2$   &$12.4\pm1.1$   \\
        %Thermal                             & -                         & $10.2982\pm0.7390$  & $10.5844\pm1.2848$  &$19.1351\pm2.5188$   & $19.2785\pm2.4635$  &$10.9877\pm1.1452$     &$12.6883\pm0.9425$   &$11.0579\pm0.1974$   &$12.3867\pm1.0605$   \\
        \midrule
        Bimodal                        & \multirow{2}{*}{Attention}     &$4.4\pm0.9$.   &$3.7\pm0.4$    &$6.5\pm0.5$    &$5.5\pm0.3$    &$5\pm1$        &$3.96\pm0.6$   &$5\pm1$        &$4.1\pm0.6$   \\
        %Bimodal                        & \multirow{2}{*}{Attention}     &$4.4245\pm0.8536$.   &$3.6854\pm0.4439$    &$6.5105\pm0.4781$    &$5.4820\pm0.2519$    &$4.9912\pm0.9701$        &$3.9625\pm0.5937$   &$5.0333\pm0.9539$        &$4.0534\pm0.6088$   \\
        Trimodal                &                                       &$4.3\pm0.4$.   &$4.2\pm1.2$    &$5.8\pm0.8$    &$5.5\pm1.5$    &$3.9\pm1.1$    &$3.6\pm1$      &$4.1\pm1$      &$3.7\pm1.1$   \\\hline
        %Trimodal                &                                       &$4.2772\pm0.3825$.   &$4.1689\pm1.1906$    &$5.8456\pm0.8186$    &$5.4675\pm1.4585$    &$3.9439\pm1.1156$    &$3.5859\pm0.9777$      &$4.0666\pm1.0344$      &$3.6522\pm1.0619$   \\\hline
        Bimodal                        & \multirow{2}{*}{ScoreAve}      &$2.1211$       &$1.9697$       &$4.8368$       &$3.4069$       &$3.0579$       &$1.5195$       &$3.5000$       &$1.8831$   \\
        %Bimodal                        & \multirow{2}{*}{ScoreAve}      &$2.3948\pm0.2602$       &$2.2049\pm0.2116$       &$5.4509\pm0.7323$       &$4.4993\pm0.5550$       &$3.7035\pm0.1160$       &$2.9807\pm0.1980$       &$3.7035\pm0.1160$       &$2.9807\pm0.1980$   \\
        Trimodal                &                                       &$2.2579$       &$1.5931$       &$4.3158$       &$3.0909$       &$2.5211$       &$1.3463$       &$2.8105$       &$1.6277$   \\
        %Trimodal                &                                       &$2.2561\pm0.0603$       &$1.7980/pm0.1039$       &$5.3070\pm0.8440$       &$4.5195\pm0.5486$       &$2.6479\pm0.2149$       &$2.1284\pm0.3475$       &$2.6479\pm0.2149$       &$2.1284\pm0.3475$   \\
        \bottomrule
\end{tabular}
\caption{EER (\%) performance results of different person verification systems under different conditions. \textit{Bimodal} and \textit{Trimodal} correspond to \textit{Audio-Visual} and \textit{Audio-Visual-Thermal} models respectively. \textit{valid'} and \textit{test'} represent the noisy version of evaluation sets. The noise rate in both train and evaluation sets is 30\%.}
\label{tab:results}
\end{table*}
\fi

\iffalse
\subsection{Robustness Evaluation}
Compare clean-noisy and noisy-noisy for trimodal and bimodal systems.

\begin{table*}[htb]
\centering
%\renewcommand\arraystretch{1.1}
%\setlength{\tabcolsep}{1.1mm}
    \begin{tabular}{l|c|cc|cc|cc}
        \toprule
        \multirow{2}{*}{Modality}       & \multirow{2}{*}{Fusion}   &   \multicolumn{2}{c|}{\scell{train clean /\\evaluation clean}}& \multicolumn{2}{c|}{\scell{train clean /\\evaluation noisy}}             & \multicolumn{2}{c}{\scell{train noisy /\\evaluation noisy}} \\\cline{3-8}
                                        &                           &  valid                        & test                          & valid             & test                     & valid                     & test                    \\ 
        \midrule
        Audio                           & -                         & $10.82\pm0.39$                & $9.29\pm0.15$                 & $18.04\pm0.26$    & $16.71\pm0.41$                                           & $14.89\pm0.60$            & $11.83\pm0.62$ \\
        %Audio                               & -                         & $10.8176\pm0.3911$  & $9.2944\pm0.1498$   & $18.0386\pm0.2579$     & $16.7056\pm0.4095$  &$12.7561\pm0.5744$   &$9.54820\pm0.3790$    &$14.8895\pm0.6035$   &$11.8312\pm0.6236$   \\
        Visual                          & -                         & $4.04\pm0.89$                 & $4.09\pm0.86$                 & $6.90\pm1.44$     & $6.56\pm1.63$                                            & $5.32\pm0.63$             & $4.38\pm0.29$ \\
        %Visual                              & -                         & $4.0439\pm0.8883$     & $4.0923\pm0.8648$   &$6.9070\pm1.4377$    & $6.5613\pm1.6331$   &$5.7632\pm0.5299$    &$4.2078\pm0.0697$      &$5.3211\pm0.6328$    &$4.3766\pm0.2896$   \\
        Thermal                         & -                         & $10.30\pm0.74$                & $10.58\pm1.28$                & $19.14\pm2.52$    & $19.28\pm2.46$                                           & $11.06\pm0.20$            & $12.39\pm1.06$ \\
        %Thermal                             & -                         & $10.2982\pm0.7390$  & $10.5844\pm1.2848$  &$19.1351\pm2.5188$   & $19.2785\pm2.4635$  &$10.9877\pm1.1452$     &$12.6883\pm0.9425$   &$11.0579\pm0.1974$   &$12.3867\pm1.0605$   \\
        \midrule
        \multirow{2}{*}{Bimodal}        & Attention                 & $4.42\pm0.85$                 & $3.69\pm0.44$                 & $6.51\pm0.48$     & $5.48\pm0.25$                                            & $5.03\pm0.95$             & $4.05\pm0.61$ \\
                                        & ScoreAve                  & $2.39\pm0.42$                 & $2.20\pm0.58$                 & $5.45\pm0.89$     & \textbf{4.50 $\pm$ 1.05}                             & $3.70\pm0.35$             & $2.65\pm0.34$ \\\cline{2-8}
        %Bimodal                        & \multirow{2}{*}{Attention}     &$4.4245\pm0.8536$.   &$3.6854\pm0.4439$    &$6.5105\pm0.4781$    &$5.4820\pm0.2519$    &$4.9912\pm0.9701$        &$3.9625\pm0.5937$   &$5.0333\pm0.9539$        &$4.0534\pm0.6088$   \\
        \multirow{2}{*}{Trimodal}       & Attention                 & $4.28\pm0.38$                 & $4.17\pm1.19$                 & $5.85\pm0.82$     & $5.47\pm1.46$                                            & $4.07\pm1.03$             & $3.65\pm1.06$ \\
        %Trimodal                &                                       &$4.2772\pm0.3825$.   &$4.1689\pm1.1906$    &$5.8456\pm0.8186$    &$5.4675\pm1.4585$    &$3.9439\pm1.1156$    &$3.5859\pm0.9777$      &$4.0666\pm1.0344$      &$3.6522\pm1.0619$   \\\hline
        %Bimodal                         & \multirow{2}{*}{ScoreAve} & $2.39\pm0.42$                 & $2.20\pm0.58$                 & $5.45\pm0.89$     & \textbf{4.50 $\pm$ 1.05}                             & $3.70\pm0.35$             & $2.65\pm0.34$ \\
        %Bimodal                        & \multirow{2}{*}{ScoreAve}      & $2.3948\pm0.2602$       & $2.2049\pm0.2116$       & $5.4509\pm0.7323$       &$4.4993\pm0.5550$       &$3.7035\pm0.1160$       &$2.9807\pm0.1980$       &$3.7035\pm0.1160$       & $2.9807\pm0.1980$   \\
                                        & ScoreAve                  & \textbf{2.26 $\pm$ 0.10}      & \textbf{1.80 $\pm$ 0.31}      & \textbf{5.31 $\pm$ 0.86}  & $4.52\pm0.59$                           & \textbf{2.98 $\pm$ 0.20}  & \textbf{2.13 $\pm$ 0.51} \\
        %Trimodal                &                                       &$2.2561\pm0.0603$       &$1.7980/pm0.1039$       & $5.3070\pm0.8440$       &$4.5195\pm0.5486$       &$2.6479\pm0.2149$       &$2.1284\pm0.3475$       & $2.6479\pm0.2149$       & $2.1284\pm0.3475$   \\
        \bottomrule
\end{tabular}
\caption{EER (\%) performance results (mean $\pm$ std) of person verification systems under three conditions: 1) \textit{train clean / evaluation clean}, 2) \textit{train clean / evaluation noisy}, and 3) \textit{train noisy / evaluation noisy}. \textit{Bimodal} and \textit{Trimodal} correspond to \textit{Audio-Visual} and \textit{Audio-Visual-Thermal} models respectively. The noise rate in both train and evaluation sets is 30\%.}
\label{tab:results}
\end{table*}
\fi


==> Odyssey 2022 Latex Template/7_conclusion.tex <==
In this work, we explored multimodal learning for the person verification task using audio, visual and thermal data streams.
We adapted the SpeakingFaces dataset to build state-of-the-art deep learning-based models.
Specifically, we developed unimodal, bimodal, and trimodal verification systems and compared their performance on easy and hard evaluation lists under the clean and noisy data conditions.
Although the visual modality achieved the best result among the unimodal systems, the audio was superior in distinguishing subjects of opposite gender.
We also observed that the thermal modality performed better than the audio modality in differentiating between subjects of the same gender.
For the multimodal systems, we compared two popular fusion strategies based on simple score averaging and the soft attention mechanism.
%We also compared two popular fusion strategies based on the simple score averaging and the attention mechanism.
%The score averaging based audio-visual-thermal verification system was found to result in remarkable performance gain over the unimodal systems, i.e., X\%, Y\% and Z\%  relative EER improvement over audio only, video only, and thermal only systems, respectively.
%The score averaging based audio-visual-thermal verification system was found to result in substantial performance gain over the unimodal systems.
The former achieved a substantial performance gain for the trimodal system compared to the other systems.
%Specifically, 55\% and 51\% relative EER improvement over the visual-based system under both conditions, respectively.
%Specifically,  55\% and 51\% relative EER improvement over the visual-based system, 18\% and 19\% relative EER improvement over the audio-visual system under clean and noisy data conditions, respectively.
Specifically, the relative EER improvements over the visual-based system were 56\% and 51\%, and 18\% and 20\% over the audio-visual system, under the clean and noisy data conditions, respectively.
%Specifically, under the clean condition, X\%, Y\% and Z\% relative EER improvement over audio, visual, and thermal systems, respectively.
%Under the noisy condition, X\%, Y\% and Z\% relative EER improvement over audio, visual, and thermal systems, respectively.
%Furthermore, the trimodal model reached 18\% and 19\% relative EER improvement over the audio-visual system under the clean and noisy conditions, respectively.
%Importantly, the integration of thermal system further boosts the robustness of person verification system, where X\% relative EER improvement over the audio-visual bimodal system is achieved on the noisy evaluation set.

In the future, we plan to thoroughly analyze the errors made by the different unimodal systems to identify the weaknesses and strengths of each modality.
We also plan to implement more advanced attention mechanisms and study the impact of different data augmentation techniques.
The robustness evaluation of multimodal verification systems at different noise rates is also a topic for future work.
